Scheduled Knowledge Acquisition on Lightweight Vector Symbolic Architectures for Brain-Computer Interfaces

Brain-Computer interfaces (BCIs) are typically designed to be lightweight and responsive in real-time to provide users timely feedback. Classical feature engineering is computationally efficient but has low accuracy, whereas the recent neural networks (DNNs) improve accuracy but are computationally expensive and incur high latency. As a promising alternative, the low-dimensional computing (LDC) classifier based on vector symbolic architecture (VSA), achieves small model size yet higher accuracy than classical feature engineering methods. However, its accuracy still lags behind that of modern DNNs, making it challenging to process complex brain signals. To improve the accuracy of a small model, knowledge distillation is a popular method. However, maintaining a constant level of distillation between the teacher and student models may not be the best way for a growing student during its progressive learning stages. In this work, we propose a simple scheduled knowledge distillation method based on curriculum data order to enable the student to gradually build knowledge from the teacher model, controlled by an $\alpha$ scheduler. Meanwhile, we employ the LDC/VSA as the student model to enhance the on-device inference efficiency for tiny BCI devices that demand low latency. The empirical results have demonstrated that our approach achieves better tradeoff between accuracy and hardware efficiency compared to other methods.

==> contents/Tables/app-cur-x11.tex <==
\begin{table}
    \setlength\intextsep{0pt}
    \setlength\lineskip{0pt}
    \captionsetup{width=\linewidth}
    \caption{Accuracy of using different $\alpha$ setups and curriculum on the X11 and S4b dataset.  }
    \centering
    \resizebox{\textwidth}{!}{
    \setlength{\tabcolsep}{10pt}
    \begin{tabular}{ccccc}
    \toprule
   
      & Static $\alpha$ & Linear $\alpha$ Scheduler & \textbf{Expo $\alpha$ Scheduler} & param $\alpha$\\
    \midrule
    
    \textbf{Curriculum KD-LDC} & \bacc{70.47}{0.67}  & \bacc{71.23}{0.84} & \bacc{71.83}{0.77} & \bacc{63.62}{0.43}\\
     KD-LDC &  \acc{69.68}{0.73} & \acc{71.03}{0.81} & \acc{71.32}{0.75} & \acc{60.99}{0.44}\\
    Anti-curriculum KD-LDC & \acc{65.89}{0.94}& \acc{66.12}{1.06} & \acc{66.34}{1.03} & \acc{56.66}{0.57}\\

    \midrule
    \midrule
    \textbf{Curriculum LDC} & \multicolumn{3}{c}{\bacc{69.19}{0.93}}\\
    LDC & \multicolumn{3}{c}{\acc{69.16}{1.04}}\\
    Anti-curriculum LDC & \multicolumn{3}{c}{\acc{65.71}{1.26}}\\


    \bottomrule
    \end{tabular}
    }

    \label{tab:app-cur-x11}
\end{table}





==> contents/Tables/app-ern-res.tex <==
\begin{table}
    \setlength\intextsep{0pt}
    \setlength\lineskip{0pt}
    \captionsetup{width=\linewidth}
    \caption{Accuracy of using different $\alpha$ setups and curriculum on the ERN dataset. }
    \centering
    \resizebox{\textwidth}{!}{
    \setlength{\tabcolsep}{10pt}
    \begin{tabular}{ccccc}
    \toprule
   
      & Static $\alpha$ & Linear $\alpha$ Scheduler & Expo $\alpha$ Scheduler & param $\alpha$\\
    \midrule
    
    \textbf{Curriculum KD-LDC} & \bacc{74.58}{0.51} & \bacc{75.19}{0.88} & \bacc{75.57}{0.62} & \bacc{69.62}{0.52}\\
    
     KD-LDC & \acc{73.86}{0.73} & \acc{74.16}{0.84} & \acc{74.87}{0.65} & \acc{68.02}{0.63}\\
     
    Anti-curriculum KD-LDC & \acc{70.06}{0.78} & \acc{70.13}{0.77} & \acc{70.20}{0.75} & \acc{66.54}{0.77} \\

    \midrule
    \midrule
    \textbf{Curriculum LDC} & \multicolumn{3}{c}{\bacc{73.35}{0.69}}\\
    LDC & \multicolumn{3}{c}{\acc{73.34}{0.87}}\\
    Anti-curriculum LDC & \multicolumn{3}{c}{\acc{69.76}{0.91}}\\


    \bottomrule
    \end{tabular}
    }

    \label{tab:app-cur-ern}
\end{table}





==> contents/Tables/app-other-student.tex <==
\begin{table*}[h]
    \setlength\intextsep{0pt}
    \setlength\lineskip{0pt}
    \captionsetup{width=\linewidth}
    \caption{Accuracy of distilling to LDC vs. other student models using different KD strategies. }
    \centering
    \resizebox{0.9\textwidth}{!}{
    \setlength{\tabcolsep}{14pt}
    \begin{tabular}{ccc}
    \toprule
   
    Dataset & Method & Accuracy  \\
     & & (\%)  \\
    \midrule
    \midrule
     \multirow{12}{*}{\textbf{Motor Imagery}} 
        
       & KD $\rightarrow$ {Binarized-DeepConvNet} &  \acc{58.13}{1.95} \\
       & KD $\rightarrow$  {Binarized-EEGNet} &  \acc{55.16}{2.01} \\ 
       & KD $\rightarrow$  {LDC} &  \acc{77.89}{0.73}\\
     
       \cmidrule(lr{1em}){2-3}
        & \textbf{ESKD} $\rightarrow$ {Binarized-DeepConvNet} &  \bacc{58.52}{2.01} \\
       & ESKD $\rightarrow$  {Binarized-EEGNet} & \acc{56.09}{1.86}  \\ 
       & ESKD $\rightarrow$  {LDC} &  \acc{79.23}{0.44} \\
       \cmidrule(lr{1em}){2-3}
        & CTKD $\rightarrow$ {Binarized-DeepConvNet} &  \acc{58.29}{2.03}\\
       & CTKD $\rightarrow$  {Binarized-EEGNet} & \acc{56.73}{1.97}\\ 
       & CTKD $\rightarrow$  {LDC} & \acc{78.85}{0.62} \\
       \cmidrule(lr{1em}){2-3}
        & ScheduledKD $\rightarrow$ Binarized-DeepConvNet &  \acc{58.36}{1.77}\\
       & \textbf{ScheduledKD} $\rightarrow$  Binarized-EEGNet & \bacc{56.88}{1.83} \\ 
       &  \textbf{\ouralg} & \bacc{80.17}{0.83} \\
    \midrule
   
    \multirow{12}{*}{\textbf{X11 and S4b}} 
        
    & KD $\rightarrow$ {Binarized-DeepConvNet}   & \acc{58.69}{1.86} \\
       & KD $\rightarrow$  {Binarized-EEGNet}   &  \acc{56.94}{1.75}\\ 
       & KD $\rightarrow$  {LDC} & \acc{69.68}{0.83}  \\
     
       \cmidrule(lr{1em}){2-3}
        & ESKD $\rightarrow$ {Binarized-DeepConvNet} & \acc{59.93}{1.27}  \\
       & ESKD $\rightarrow$  {Binarized-EEGNet}   & \acc{58.21}{0.86}\\ 
       & ESKD $\rightarrow$  {LDC} & \acc{71.19}{1.04}\\
       \cmidrule(lr{1em}){2-3}
        & CTKD $\rightarrow$ {Binarized-DeepConvNet} &  \acc{59.74}{1.31} \\
       & CTKD $\rightarrow$  {Binarized-EEGNet}   & \acc{58.83}{0.97}\\ 
       & CTKD $\rightarrow$  {LDC}   &   \acc{70.22}{0.64}\\
       \cmidrule(lr{1em}){2-3}
        & \textbf{ScheduledKD} $\rightarrow$ Binarized-DeepConvNet   &  \bacc{60.27}{0.84}\\
       & \textbf{ScheduledKD} $\rightarrow$  Binarized-EEGNet &  \bacc{58.90}{0.92} \\ 
       &  \textbf{\ouralg} & \bacc{71.83}{0.77}  \\
    
     \midrule
     \multirow{12}{*}{\textbf{ERN}} 
        
       & KD $\rightarrow$ {Binarized-DeepConvNet}   & \acc{61.88}{0.75}\\
       & KD $\rightarrow$  {Binarized-EEGNet}   & \acc{60.16}{1.54}\\ 
       & KD $\rightarrow$  {LDC}   & \acc{73.86}{0.73}\\
     
       \cmidrule(lr{1em}){2-3}
        & ESKD $\rightarrow$ {Binarized-DeepConvNet} &  \acc{62.87}{1.08} \\
       & ESKD $\rightarrow$  {Binarized-EEGNet}   & \acc{61.17}{1.23}\\ 
       & ESKD $\rightarrow$  {LDC}  & \acc{75.03}{0.66} \\
       \cmidrule(lr{1em}){2-3}
        & CTKD $\rightarrow$ {Binarized-DeepConvNet} &  \acc{62.88}{0.71} \\
       & CTKD $\rightarrow$  {Binarized-EEGNet} &  \acc{61.15}{0.79} \\ 
       & CTKD $\rightarrow$  {LDC} &   \acc{74.42}{0.60} \\
       \cmidrule(lr{1em}){2-3}
        & ScheduledKD $\rightarrow$ Binarized-DeepConvNet &  \bacc{63.47}{0.79} \\
       & ScheduledKD $\rightarrow$  Binarized-EEGNet & \bacc{61.53}{0.91}  \\ 
       &  \textbf{\ouralg} & \bacc{75.57}{0.62}  \\

    \bottomrule
    \end{tabular}
    }
    \label{tab:app-other}

\end{table*}





==> contents/Tables/app-params.tex <==
\begin{table}
    \caption{Other hyperparameters values. Note that the value of $\alpha$ listed here in the \ouralg method is the starting value.}
    \centering
    \resizebox{1\textwidth}{!}{
    \setlength{\tabcolsep}{14pt}
    \begin{tabular}{llp{6cm}}
    \toprule
    Dataset & Method & Parameters \\
    % Dataset & Method & Parameters \\
    \midrule
    \multirow{4}{*}{\textbf{Motor Imagery}} &  
    % EEGNet &  lr:  \\
    % & DeepConvNet &  \\
    % & Binarized-DeepConvNet &  \\
    % & SVM &   \\
    % & MLP &    \\
    % & LeHDC &   \\
    % & LDC &   \\
     KD-LDC & $\alpha: 0.1$\quad $\tau: 5$\\
    & ESKD w/ LDC & $\alpha: 0.1$\quad $\tau: 5$\\
    & CTKD w/LDC & $\alpha: 0.05$\quad $\tau: 5$ \\
 
    & \ouralg & $\alpha: 0.5$\quad $\tau: 5$\quad $\gamma: 0.96$\quad $r: 10$\\
   
    \midrule
    \multirow{4}{*}{\textbf{X11 and S4b}} 
    % &  EEGNet &   \\
    % & Binarized-EEGNet & \\
    % & DeepConvNet &   \\
    % & SVM &    \\
    % & LeHDC &   \\
    % & LDC &    \\
    & KD-LDC & $\alpha: 0.2$\quad $\tau: 10$\\
    & ESKD w/ LDC & $\alpha: 0.2$\quad $\tau: 10$; \\
    & CTKD w/LDC & $\alpha: 0.1$\quad $\tau: 8$ \\
 
    & \ouralg & $\alpha: 0.1$\quad $\tau: 8$\quad $\gamma: 0.90$\quad $r: 10$\\
  
    \midrule
   \multirow{4}{*}{\textbf{ERN}} &  
   %  EEGNet &  \\
   % & Binarized-EEGNet &  \\
   %  & DeepConvNet &    \\
   %  & SVM &   \\
   %  & LeHDC &    \\
   %  & LDC &  \\
     KD-LDC & $\alpha: 0.1$\quad $\tau: 10$\\
    & ESKD w/ LDC & $\alpha: 0.15$\quad $\tau: 10$ \\
    & CTKD w/LDC & $\alpha: 0.1$\quad $\tau: 10$ \\
 
    & \ouralg & $\alpha: 0.1$\quad $\tau: 10$\quad $\gamma: 0.96$\quad $r: 10$\\
    \bottomrule
    \end{tabular}
    }
    \label{tab:params}
\end{table}
